Let's Negotiate! A Survey of Negotiation Dialogue Systems

Negotiation is one of the crucial abilities in human communication, and there has been a resurgent research interest in negotiation dialogue systems recently, which goal is to empower intelligent agents with such ability that can efficiently help humans resolve conflicts or reach beneficial agreements. Although there have been many explorations in negotiation dialogue systems, a systematic review of this task has to date remained notably absent. To this end, we aim to fill this gap by reviewing contemporary studies in the emerging field of negotiation dialogue systems, covering benchmarks, evaluations, and methodologies. Furthermore, we also discuss potential future directions, including multi-modal, multi-party, and cross-cultural negotiation scenarios. Our goal is to provide the community with a systematic overview of negotiation dialogue systems and to inspire future research.

==> 9-related_work.tex <==
\section{Related Work}

other relevant survey work on dialogue systems.

==> negotiation survey/1-introduction.tex <==


\section{Introduction}

% \begin{quote}
%     ``"
%     \qauthor{\textit{}}
% \end{quote}

\epigraph{\textit{``Let us never negotiate out of fear. But let us never fear to negotiate.''}}{\textit{John F. Kennedy}}

%Negotiation is a common strategic communication between two or more people to resolve points of difference, gain an advantage for an individual or collective, or craft outcomes to satisfy various interests~\cite{}. It is pervasive in human daily interaction, which occurs when people communicate to manage conflict or make compromises. An agent that can understand human language and negotiate logically, would significantly benefit human society, from bargaining prices to high-stake political or legal situations. 

Negotiation is one of the crucial abilities in  human communication that involves two or more individuals discussing goals and tactics to resolve conflicts, achieve mutual benefit, or find mutually acceptable solutions~\cite{fershtman1990importance,bazerman1993negotiating,lewicki2011essentials}. It is a common aspect of human interaction, occurring whenever people communicate in order to manage conflict or reach a compromise. Scientifically,  one of the long-term goals of dialogue research is to empower intelligent agents with such ability. Agent effectively negotiating with a human in natural language could have significant benefits in many scenarios, from bargaining prices in everyday trade-in~\cite{he2018decoupling} to high-stakes political or legal situations~\cite{basave2016study}.





\begin{figure}
    \centering  
    \includegraphics[width=0.49\textwidth]{images/intro.pdf}
    \caption{The negotiation process involves a multi-turn interaction between agent and human. They exchange information about their deals and end up with accepting or declining deals.}
    \label{fig:intro}
\end{figure}

Negotiation dialogue systems~\cite{lewandowska1982meaning,lambert1992modeling,chawla2021casino} is an emerging research field that aims to build intelligent conversational agents that can automatically negotiate with a human in natural languages, e.g., CICERO\footnote{\url{https://ai.facebook.com/research/cicero/}} from Meta AI. Agents negotiate with human through multi-turn interaction using logically reasoning~\cite{sycara2010agent} over  goals~\cite{zhang2020learningbebavior}, strategies~\cite{zhou2019augmenting} and psychology factors~\cite{yang2021improving}. As illustrated in Figure~\ref{fig:intro}, negotiation dialogue agents interact with the human through multi-turn cycles.
A successful negotiation process involves efficient information exchange, strategic discussion toward their goals, and a closing section.  

% Despite many research work has been proposed in the task, we find a comprehensive survey is missing. In this work, we propose a survey of negotiation dialogue system from benchmarks, methodology, evaluation and future directions. Various benchmarks have been proposed in the recent years, which includes different scenarios, such as bargaining, game, job interview, persuasion. We categorize these datasets based on the strategy type: distributive, such as bargaining, and integrative, such as maximizing outcomes.


Despite the significant amount of research that has been conducted on the task, there is a lack of a systematic review of the topic. In this work, we aim to fill this gap by reviewing contemporary work in the emerging field of negotiation dialogue systems, covering aspects such as benchmarks, evaluation, methodology, and future directions. In recent years, various benchmarks have been proposed for negotiation dialogue systems, ranging from bargaining~\cite{lewis2017deal} and game scenarios~\cite{stac2016discourse} to job interviews~\cite{zhou-etal-2019-dynamic} and items exchanging~\cite{chawla2021casino}. 
Our survey will provide an overview of these benchmarks and discuss how they have been used to evaluate the performance of negotiation dialogue systems.


Modeling the negotiation process for conversational agents also imposes challenges. Firstly, these agents must be able to reason about and employ various strategies in different situations. In addition to strategy modeling, it is also necessary to model the personalities (e.g., mind, emotion, and behaviors) of the negotiators. Thirdly, an effective policy learning method is essential for the successful use of language. To address these challenges, we can categorize existing solutions into three areas: (1) Personality modeling helps us understand negotiator's preferences, (2) Strategy modeling enables agents to make reasonable decisions based on gathered information, and (3) Policy learning methods utilize information effectively to maximize results.


In summary, our contributions are three-fold: (1) To the best of our knowledge, we systematically categorize current negotiation dialogue benchmarks from the perspective of distributive and integrative, with each category based on different goal types of negotiation dialogue tasks. (2) We categorize typical evaluation methods and current solutions into an appropriate taxonomy. (3) We pointed out the current limitation and promising research directions in the future.

% Outlines:

% \textbf{Paragraph 1:} broad definition of negotiation in human communication. Highlight its importance of negotiation dialogue systems. briefly introduce the function of negotiation dialogue agents.

% (e.g., Negotiation is a common strategic communication between two or more people to resolve points of difference, gain an advantage for an individual or collective, or craft outcomes to satisfy various interests~\cite{} .)

% \textbf{Paragraph 2:} Highlight the promising research value of negotiation dialogue systems (giving citation). specific definition of the task of negotiation dialogue (using a figure to illustrate if possible).


% \textbf{Paragraph 3:} Introduce the challenges that Negotiation dialogue still faces. using itemsize to list out.


% \textbf{Paragraph 4:} highlight our motivation to propose this survey. introduce the structure of following parts. 

% \textbf{Paragraph 5:} Shortly summarize our contributions.




==> negotiation survey/2-social_impact.tex <==
%\section{Social Impact}
\section{Backgrounds}

\subsection{Negotiation in Human}
%% Suraj

% concepts of negotiation,
% lay out some foundation for this concept.

% negotiation in real-world

% \subsection{Negotiation in Social Science}


% Introducing the function of negotiation in human communication from the perspective of social science, including psychology, 


% (useful reference: \cite{fershtman1990importance,bazerman1993negotiating,lewicki2011essentials,o2015persuasion})

% Framework:
% (1) Negotiation in human and its function

Humans negotiate everyday in their daily routines. Negotiation is used to manage conflict and is the primary give-and-take process by which people try to reach an agreement~\cite{fisher2011getting,lewicki2011essentials}. Research on negotiation has been conducted for almost 60 years in the field of psychology, political science, and communication. It has evolved over the past decades from exploring game theory~\cite{walton1991behavioral}, behavior decisions driven by the cognitive revolution in psychology~\cite{bazerman1993negotiating}, to cultural differences in the 2000s~\cite{bazerman2000negotiation}.
Negotiation research, however, is now forced to confront the implications of human/AI collaborations given recent advancements in machine learning~\cite{sycara2010agent}.
%(Bazerman et al., 2000; Ouali, Sabouret & Rich, 2017). 
Converging efforts from social scientists and data scientists who incorporate insights from both fields will be fruitful in maximizing expectations and outcomes during negotiation processes.


Negotiation is a process by which two or more parties attempt to resolve their opposing interests. {Strategy} of negotiation can be \textit{distributive}, such as bargaining~\cite{fershtman1990importance} and \textit{integrative}, such as maximizing unilateral interests~\cite{bazerman1993negotiating}, both of which are used in various social situations such as informal, peer to peer, organizational, and diplomatic country to country settings. The implications for enhancing outcomes are thus large and important to understand. Research from psychology demonstrates that the negotiation process can be affected by psychological factors, such as personality~\cite{sharma2013role}, relationship~\cite{olekalns2003testing}, social status~\cite{blader2012differentiating}, and cultural background~\cite{leung2011within}.  

==> negotiation survey/3-tech_background.tex <==
%\section{Backgrounds}

% from the system perspective, machine learning, NLP/AI


% definition of backgrounds


% features:

% - non-collaborative, goal-driven
% - purpose: reach an agreement
% - win-win/win-loss

%\subsection{Negotiation in Social Science}



\subsection{Task Definition}



The ability of an agent to maintain good communication skills as well as strategic reasoning capabilities is what makes a negotiation dialogue system unique from typical task-oriented and open-domain systems. Negotiation dialogue aims to interact with opponents in a strategic discussion to find acceptable solutions for both parties. A negotiation process involves a mixture of strategies such as debate, persuasion, adversary, and compromise. These strategies will change along with the negotiation flow and can be influenced by opponents' personalities (e.g., thoughts, emotions, and behaviors). Therefore, \textbf{strategy} and \textbf{personality} are two main aspects to be modeled in negotiation dialogue systems. Formally, a negotiation dialogue task is defined as a tuple $(\mathcal{K}, \mathcal{S}, \mathcal{U}, \pi, {g})$. $\mathcal{K}$ refers to the pre-defined information which is prepared for the negotiation process, such as the negotiator's preferences and demands. $\mathcal{S}$ refers to a trajectory $\{s_1, s_2, ...\}$, which is used to model the strategy transition process and provided for policy learning module (e.g., reinforcement learning). A series turn of dialogue interactions $\mathcal{U}$ can be viewed as $\{u_1, u_2, ...\}$ are generated along with the negotiation process. A policy learning module $\pi_{\theta}(\mathcal{K}, \mathcal{S}, \mathcal{U})$ is utilized to learn an optimal deterministic policy which helps reach the negotiation goal $g$.



%\subsection{Negotiation Dialogue v.s. Others}

%Difference and overlap between negotiation dialogues and chit-chat dialogues.


==> negotiation survey/4-dataset.tex <==
\section{Negotiation Datasets}
\label{datasetsection}
\begin{table*}[t]
\begin{center}
\small
\setlength{\tabcolsep}{1.6mm}{
\begin{tabular}{lccccc}
\toprule
DataSet & Negotiation Type & Scenario & \# Dialogue  & \# Avg. Turns & \# Party \\
\midrule
InitiativeTaking (\citeyear{nouri-traum-2014-initiative}) & Integrative & Fruit Assignment & 41  & - & Multi\\
STAC (\citeyear{stac2016discourse}) & Integrative & Strategy Games & 1081 & 8.5  & Two \\
DealorNoDeal (\citeyear{lewis2017deal}) & Integrative & Item Assignment & 5808 & 6.6 & Two \\
Craigslist (\citeyear{he2018decoupling}) & Distributive & Price Bargain & 6682 & 9.2 & Two \\
NegoCoach (\citeyear{zhou-etal-2019-dynamic}) & Distributive & Price Bargain & 300 & - & Two \\
PersuasionforGood (\citeyear{wang-etal-2019-persuasion}) & Distributive & Donation & 1017 & 10.43 & Two \\
FaceAct (\citeyear{dutt2020keeping}) & Distributive & Donation & 299 & 35.8 & Two\\
AntiScam (\citeyear{li2020end}) & Distributive & Privacy Protection & 220  & 12.45 & Two\\
CaSiNo (\citeyear{chawla2021casino}) & Integrative & Item Assignment & 1030 & 11.6 & Two \\
JobInterview (\citeyear{yamaguchi-etal-2021-dialogue}) & Integrative & Job Interview & 2639 & 12.7 & Two \\
DinG (\citeyear{boritchev-amblard-2022-multi}) & Integrative & Strategy Games & 10 & 2357.5 & Multi \\
\bottomrule
\end{tabular}}
\caption{Negotiation dialogues benchmarks are sorted by their publication time. For each dataset, we introduce the negotiation type, scenario, the number of dialogues and corresponding average turns, and party attributes.}
\label{tab:dataset}
\end{center}
\end{table*}
In this section, we summarize the existing negotiation datasets and resources. 
Table~\ref{tab:dataset} shows all of the collected benchmarks, along with their negotiation types, scenarios and data scale. In this paper, we categorize these benchmarks based on their negotiation types, namely, \textit{integrative} negotiation and \textit{distributive} negotiation. The integrative negotiation is associated with win-win scenarios, and its goal is to develop mutual gain. On the contrary, the distributive negotiation is often associated with win-lose scenarios and aims to maximize personal benefits. In general, The distributive negotiation is more competitive than its integrative counterpart. 


\subsection{Integrative Negotiation Datasets}
In integrative negotiations, there is normally more than one issue available to be negotiated. To achieve optimal negotiation goals, the involved players should make trade-offs for multiple issues.

\paragraph{Multi-player Strategy Games} The strategy video games provide ideal platforms for people to verbally communicate with other players to accomplish their missions and goals.~\citet{stac2016discourse} propose the STAC benchmark, which is the player dialogue in the game of Catan. In this game, players need to gather resources, including wood, wheat, sheep, and more, with each other to purchase settlements, roads and cities. As each player only has access to their own resources, they have to communicate with each other. To investigate the linguistic strategies used in this situation, STAC also includes an SDRT-styled discourse structure. \citet{boritchev-amblard-2022-multi} also collect a \emph{DinG} dataset  from French-speaking players in this game. The participants are instructed to focus on the game, rather than talk about themselves. As a result, the collected dialogues can better reflect the negotiation strategy used in the game process.


\paragraph{Negotiation for Item Assignment}
The item assignment scenarios involve a fixed set of items as well as a predefined priority for each player in the dialogue. As the players only have access to their own priority, they need to negotiate with each other to exchange the items they prefer. \citet{nouri-traum-2014-initiative} propose \emph{InitiativeTalking}, occurring between the owners of two restaurants. They discuss how to distribute the fruits (i.e., apples, bananas, and strawberries) and try to reach an agreement. \citet{lewis2017deal} propose \emph{DealorNoDeal}, a similar two-party negotiation dialogue benchmark where both participants are only shown their own sets of items with a value for each and both of them are asked to maximize their total score after negotiation. \citet{chawla2021casino} propose \emph{CaSiNo}, a dataset on campsite scenarios involving campsite neighbors negotiating for additional food, water, and firewood packages. Both parties have different priorities over different items.

\paragraph{Negotiation for Job Interview}
Another commonly encountered negotiation scenario is job offer negotiation with recruiters. \citet{yamaguchi-etal-2021-dialogue} fill this gap and propose the \emph{JobInterview} dataset. JobInterview includes recruiter-applicant interactions over salary, day off, position, company, and workplace. The participants are shown negotiators’ preferences and the corresponding issues and options and are given feedback in the middle of the negotiation.

\subsection{Distributive Negotiation Datasets}
Distributive negotiation is about the discussion over a fixed amount of value (i.e., slicing up the pie). In such negotiation, the involved people normally talk about a single issue (e.g., item price) and therefore, there are hardly trade-offs between multiple issues in such negotiation. 

\paragraph{Persuasion For Donation}
Persuasion, convincing others to take specific actions, is a necessary required skill for negotiation dialogue~\cite{sycara1990persuasive,sierra1997framework}. \citet{wang-etal-2019-persuasion} focus on persuasion and propose \emph{PersuasionforGood}, a two-party persuasion conversations about charity donations. In the data annotation process, the persuaders are provided some persuasion tips and example sentences, while the persuaders are only told that this conversation is about charity. The annotators are required to complete at least ten utterances in a dialogue and are encouraged to reach an agreement at the end of the conversations. \citet{dutt2020keeping} further extend \emph{PersuasionforGood} by adding the utterance-level annotations that change the positive and/or the negative face of the participants in a conversation. A face act can either raise or attack the positive face or negative face of either the speaker or the listener in the conversation. 


\paragraph{Negotiation For Product Price}
Negotiations over product prices can be observed on a daily basis. 
\citet{he2018decoupling} propose \emph{CraigslistBargain}, a negotiation benchmark based on a realistic item price bargaining scenario. In \emph{CraigslistBargain}, two agents, a buyer and a seller, are required to negotiate the price of a given item. The listing price is available to both sides, but the buyer has a private price as the target. Then two agents chat freely to decide the final price. The conversation is completed when both agents agree with the price or one of the agents quits. \citet{zhou-etal-2019-dynamic} propose \emph{NegoCoach} benchmark on similar scenarios, but with an additional negotiation coach who monitors messages between the two annotators and recommends tactics in real-time to the seller to get a better deal.


\paragraph{User Privacy Protection}
Privacy protection of negotiators has become more and more vital. Participant (e.g., attackers and defenders) goals are also conflicting. \citet{li2020end} propose \emph{Anti-Scam} benchmark which focuses on online customer service. In \emph{Anti-Scam}, users try to defend themselves by identifying whether their components are attackers who try to steal sensitive personal information. \emph{Anti-Scam} provides an opportunity to study human elicitation strategies in this scenario. 

==> negotiation survey/5-modeling_method.tex <==
\section{Methodology Overviews}

%\textbf{Framework 1:} Research problem oriented

As shown in Figure~\ref{fig:method}, we categorize existing methods into \emph{Strategy Modeling}, \emph{Personality Modeling}, and \emph{Policy Learning}. Strategy modeling methods help conversational agents utilize appropriate strategies in different situations. In addition, negotiation is not only about complex reasoning over strategies,  but also influenced by psychology factors. Personality is one of the most important psychology factors that would affect agents' decisions. Therefore, personality modeling helps agents perceive opponents. Besides, an effective policy
learning method is indispensable for the successful use of language.

%Besides, policy learning helps agents learn in a good format. 


\begin{figure}
    \centering
    \includegraphics[width=0.49\textwidth]{images/method.pdf}
    \caption{A summary of different methods proposed by previous research efforts for the negation dialogues.}
    \label{fig:method}
\end{figure}


\subsection{Strategy Modeling}


% \haolan{Outlines: (Haolan's suggestion)  \\
% (1) Principled / Integrative / Win-win;\\
% (2) Adversarial / Distributive / Win-loss; \\
% (3) Multi-party;\\
% (4) Team Negotiation (No related paper).
% }

In this section, we discuss strategy modeling for negotiation dialogue systems. Negotiation strategies include a range of tactics and approaches that people use to achieve their goals in negotiation processes. It can be categorized into three aspects: \emph{integrative} (win-win) and \emph{distributive} (win-lost), and \emph{multi-party}. 
%integrative strategy is one where both parties are able to achieve an agreement that meets their respective needs and concerns. For example, a buyer and a seller are trying to reach an agreement on the price of a product. In this situation, the buyer might want to pay as little as possible for the product, while the seller wants to sell with highest price. To reach an agreement that benefit both sides, the buyer and seller can try to find a middle ground where both parties are satisfied. In contrast, competitive strategy is one where one party attempts to gain an advantage over the other. This type of negotiation can often be adversarial, because each party tries to get the best deal for themselves at the expense of the other. For example, in a situation that two companies bidding for a contract to provide a product or service to a third party, one company might offer a lower price, while the other might offer additional features or benefits. The goal in this case would be to outcompete the other company and win the contract, even if it means sacrificing some profit. Most negotiation strategies in negotiation dialogue system can be divided into collaborative strategy or competitive strategy.

\subsubsection{Integrative Strategy}
Integrative strategy (known as \emph{win-win}) modeling aims to achieve mutual gain among participants. For instance, \citet{zhao2019rethinking} proposes to model the discourse-level strategy using a latent action reinforcement learning (LaRL) framework. LaRL can model strategy transition within a latent space. However, due to the lack of explicit strategy labels, LaRL can only analysis strategies in implicit space. To resolve the problem, \citet{chawla2021casino} define a series of explicit strategies such as \emph{Elicit-Preference}, \emph{Coordination} and \textit{Empathy}. While \textit{Elicit-Preference} is a strategy attempting to discover the preference of the opponent, \textit{Coordination}  promotes mutual benefits by explicit offer or implicit suggestion. 
In order to capture user's preference, \citet{chawla2022opponent} utilize those strategies using a hierarchical neural model. Besides, \citet{yamaguchi2021dialogue} present another collaborative strategy set to negotiate workload and salaries during the interview, which goal is to reach an agreement between employer and employee. It assists humans in becoming better negotiators during this process, e.g., communicating politely, addressing concerns, and providing side offers.



%which is an attempt to express positive acknowledgement to a personal context of the partner,  to build a rapport with the partner.  \textit{Coordination}  promotes mutual benefits by explicit offer or implicit suggestion. \textit{Elicit-Preference} attempts to discovery the preference of the opponent. \cite{zhou-etal-2019-dynamic} proposed more explicit behavior for collaborative strategy. For example, to build a trust, they suggested communicating with opponent politely and deepening interpersonal relationship. To promote mutual gain, negotiator can offer side offers, communicate your interests or address opponent's concern. 

\subsubsection{Distributive Strategy}
Distributive strategy (known as \emph{win-loss}) modeling focuses on achieving one's own goals and maximizing unilateral interests more than mutual benefits. Distributive strategy can be used when you insist on your position or resist the opponent's deal~\cite{zhou-etal-2019-dynamic}. For example, \citet{dutt-etal-2021-resper} investigate four resisting categories, namely contesting, empowerment, biased processing, and avoidance \cite{fransen2015strategies}. Each individual category contains fine-grain strategic behaviors. For example, contesting refers to attacking the message source, and empowerment implies reinforcing personal preference to contradict a claim (\textit{Attitude Bolstering}) or attempting to arouse guilt in the opponent (\textit{Self Pity}). Besides, \citet{wang-etal-2019-persuasion} design a set of persuasion strategies to persuade others to donate to charity. It contains 10 different strategies containing logical appeal, emotional appeal, source-related inquiry and etc. \citet{li-etal-2020-exploring-role} explore the role structure to enhance the strategy modeling. \citet{dutt2020keeping} further enhances the role modeling with facing act, which helps utilize strategy between asymmetric roles.



%There are many specific behaviors under competitive strategy. \citet{chawla2021casino} defined \textit{Undervalue-Partner}, which undermines the requirements of their opponent, and \textit{Vouch-Fairness}, which appeals to fairness for personal benefit when the opponent offers a deal that benefit them. Competitive strategy can also be expressed by insisting on your position or resisting opponent's position\cite{zhou-etal-2019-dynamic}. \citet{dutt-etal-2021-resper} investigated four resisting categories, namely contesting, empowerment, biased processing, and avoidance \cite{fransen2015strategies}. Each individual category contains fine-grain behaviors. For example, Contesting refers to attacking the message source (\textit{Source Derogation}) or message content (\textit{Counter Argumentation}). Empowerment can be applied by reinforcing personal preference to contradict a claim (\textit{Attitude Bolstering}) or attempting to arouse guilt in the opponent (\textit{Self Pity}). Besdies, \citet{persu} 


\subsubsection{Multi-party Strategy}

While previously mentioned work on integrative and distributive strategy modeling mainly relates to two-party, multi-party strategy modeling is slightly different.  In multi-party situations, strategy modeling needs to consider different attitudes and complex relationships among individual participants, whole groups, and subgroups~\cite{traum2008multi}. \citet{georgila2014single} attempt to model multi-party negotiation using a multi-agent RL framework. Furthermore, \citet{shi2019deep} propose to construct a discourse dependency tree to predict relation dependency among multi-parties. Besides, \citet{li2021dadgraph} disclose relations between multi-parties using a graph neural network. However, due to the limited access to multi-party datasets, strategy modeling on multi-party scenarios is under-explored.

%There are many specific behaviors under competitive strategy. \citet{chawla2021casino} defined \textit{Undervalue-Partner}, which undermines the requirements of their opponent, and \textit{Vouch-Fairness}, which appeals to fairness for personal benefit when the opponent offers a deal that benefit them. Competitive strategy can also be expressed by insisting on your position or resisting opponent's position\cite{zhou-etal-2019-dynamic}. \citet{dutt-etal-2021-resper} investigated four resisting categories, namely contesting, empowerment, biased processing, and avoidance \cite{fransen2015strategies}. Each individual category contains fine-grain behaviors. For example, Contesting refers to attacking the message source (\textit{Source Derogation}) or message content (\textit{Counter Argumentation}). Empowerment can be applied by reinforcing personal preference to contradict a claim (\textit{Attitude Bolstering}) or attempting to arouse guilt in the opponent (\textit{Self Pity}). 


% \paragraph{Strategy Recognition and Next Strategy Prediction}
% Strategy recognition aims to identify the usage of negotiation strategy in the observed utterances,  while the task of next strategy prediction aims to predict possible next strategies based on conversation history. Both can be treated as multi-label classification problem as one utterance contains more than one strategy in most cases . The difference is input data. For strategy recognition, the input is an observed utterance with or without history. For next strategy prediction, the input is conversation history. 

% The classification modeling usually contain a encoding module and classification module. Encoding module converts text into continuous representation. Then, continuous representation is fed to classification module to predict strategies. For example, \citet{chawla2021casino} used a BERT-based encoder to compute contextual token representation and independent binary classifiers to predict labels. Rule-based methods are also a reliable way to recognize simple strategies \cite{zhou-etal-2019-dynamic}.


% \paragraph{Hierarchical Argumentation Structure for Persuasive Argumentative Dialogue Generation\cite{Kazuki_SAKAI20202019EDP7147}}
% This work focus on generating persuasive argumentative utterance. The system consists of a dialogue manager and natural language generator. For dialogue manager, it takes user's utterance as input. Then, it select one viewpoint and find premises to support the viewpoint, which is called argumentation. The reasoning process from viewpoint to premises is completed in a KG called AIFdb \cite{Lawrence2012AIFdbIF}. Argumentation from dialogue manager is in hierarchical structural format. To convert it to natural language, an NLG module modifies the surface text according to the ad-hoc rules. The experimental results suggested that the utterance produced by proposed hierarchical method is more persuasive than the flat structure method. 

% \paragraph{Refine and Imitate: Reducing Repetition and Inconsistency in Persuasion Dialogues via Reinforcement Learning and Human Demonstration\cite{shi-etal-2021-refine-imitate}}
% This work aims to reduce repetition and inconsistency problem in dialogue generation. They propose to use reinforcement learning to penalize repetitive and inconsistent utterance during generation. To address the limitation of real-time interaction with environment in RL, the work train a human imitator to imitate human demonstrations to select final response.

% During RL training, for each iteration, they sample one dialogue from training set. For each turn of this dialogue, a pre-trained Language model $p_{\theta}$ generates $n$ response candidates. Then a response detector annotates these candidates with labels (e.g. Strategy, Non-Strategy, Inconsistency, Repetition, etc). Candidates receive rewards  based on designed reward function, which encourage consistency and diversity. Combining with human response, which has highest reward, all generated candidates are stored in replay buffer with corresponding rewards. Finally, $p_{\theta}$ is updated from examples in replay buffer. Moreover, to prevent $p_{\theta}$ moving too far away from the original mode and potentially lose fluency, they add a KL term as an regularizer in loss function.

% During testing, after generating $n$ candidates, a response filter is in charge of remove inconsistent and repetitive candidates. Then a human imitator select the most persuasive candidates as the final output. The human imitator is trained on a collected dataset. 

% The experiment results show their model achieves state-of-the-art performance in a donation persuasion task.

% \paragraph{Reinforcement Learning of Argumentation Dialogue Policies in Negotiation\cite{georgila2011reinforcement}}
% This work use reinforcement learning for learning a negotiation policy. To learn such a policy, they design three types of simulated users (individualist, collectivist, and altruist) as environment. Those simulated users are hybrid models (partly learned neural net, partly hand-crafted). Then they define reward functions to guide updating of policy parameters. For training, they use the SARSA-$\lambda$ algorithm to explore the state-action space. The evaluation results show the policy trained with individualist simulated users perform well when tested with other types of simulated users, which is promising and expected.

% \paragraph{DialoGraph: Incorporating Interpretable Strategy-Graph Networks into Negotiation Dialogues\cite{joshi2021dialograph}}
% DialoGraph is an end-to-end negotiation dialogue system that focus on modeling negotiation strategies in negotiation dialogue. DialoGraph leverages Graph Attention Networks (GAT) \cite{velickovic2017graph} to learn the complex associations between negotiation strategies. They annotate each utterance with coarse dialogue acts (e.g. inquiry, inform, agree, etc) and fine-grained strategies (e.g. describe product, build rapport, address concerns, etc).

% DialoGraph consists of three main components: (i) utterance encoder that maps utterances to continuous representation; (ii) strategy encoder that encodes sequence of dialogue acts and negotiation strategies; (iii) utterance decoder that generate utterance based on context. 

% Evaluation results show DialoGraph reach highest performance on next dialogue-act and strategy prediction. Human evaluation present DialoGraph has best performance on persuasive, coherent and understandable.

% \paragraph{Comparing The Accuracy of Frequentist and Bayesian Models in Human-Agent Negotiation\cite{EmmanuelComparingNegotiation}}
% This work revisits the pros and cons of Bayesian and frequestist approaches to opponent modeling. Opponent modeling attends to reveal opponent's preferences during the course of a negotiation. Bayesian approaches try to infer preferences by updating probability of preference profiles based on a sequence of observations during negotiation, while frequentist approaches aim to estimate weights over preference profiles by looking at how often the one profile is offered.
% The evaluation results show that frequentist opponent models outperform Baysian models when using a uniform prior, Baysian approaches excel when using two common priors.

% \paragraph{Decoupling Strategy and Generation in Negotiation Dialogues \cite{he2018decoupling}}
% \begin{itemize}
% \item They collected negotiation dialogues dataset named CraigslistBargain, which is available here \footnote{\url{https://stanfordnlp.github.io/cocoa/}}. Comparing to other dataset, CraigslistBargain is designed to focus on more realistic scenarios. During data collection, two agents are assigned the role of a buyer and a seller; they are required to negotiate the price of a given item. As the real scenario, the listing price is available to both sides, but buyer has a private price as target. Then two agents chat freely to decide the final price. When a price is accepted  by the partner, the task is completed. Agents can also quit the conversation as no agreement completion. Furthermore, agents can negotiate side offers (e.g. free delivery or pick up) to simulate real scenarios. Statistics of CraigslistBargain are shown in Table~\ref{tab:CraigslistBargain_statistics}.
% \item They define coarse dialogue acts (e.g. greet, disagree, insist, inquire, propose, counter, etc), which serves as a logical skeleton on conversation level. Each utterance is assigned with one dialogue act.
% \item The proposed model contains three modules: a parser that maps an utterance into dialogue act; a manager that predict next dialogue act given past history; a generator that produce natural language response conditioning on past history and predicted dialogue act.
% \end{itemize}

\subsection{Personality Modeling}

% \haolan{
% Outlines: \\
% Mind/mental state modeling\\
% Emotion/Face acts modeling \\
% Behavior modeling.\\
% }
Negotiation dialogue involves complex social interactions related to multiple disciplines, such as psychology, for understanding human decision-making. Personality is an important factor in the understanding human-decision process. We summarize those work modeling personality from three perspectives: \textit{Mind}, \textit{Emotion}, and \textit{Behavior} modeling. 


\subsubsection{Mind Modeling}
Mind modeling in negotiation dialogue systems encompasses several tasks, such as mind preference estimation and opponent response prediction. Mind preference estimation helps the agent infer the intention of the opponents and guess how their own utterances would affect the opponent's mental preference. \citet{nazari2015opponent} propose a heuristic frequency-based method to estimate the negotiator's preference. \citet{langlet2018detecting} consider a rule-based system incorporating linguistic features to identify user's preference. A critical challenge for mind modeling in negotiation is that it usually requires complete dialogues, so it is difficult to predict those preferences precisely for partial dialogue. To make it applicable for those partial dialogues, which is widespread in real-world applications, \citet{chawla2022opponent} formulated mind preference estimation as a ranking task and proposed a transformer-based model that can be trained directly on partial dialogue.

In terms of opponent response prediction, \citet{he2018decoupling} firstly propose to decouple the modeling of the strategy of generation containing a parser to map utterances with dialogue acts and a dialogue manager to predict the skeleton of dialogue acts. \citet{yang2021improving} further improve the negotiation system with a first-order model based on the theory of Mind~\cite{frith2005theory} , which allows the agents to compute an expected value for each mental state. They provided two variance variants of ToM-based dialogue agents: explicit and implicit, which can fit both pipeline and end-to-end systems.


\subsubsection{Emotion Modeling}

Emotion modeling refers to recognizing the emotional change between negotiators. Therefore, explicit modeling of emotions throughout a conversation is crucial to capture reflections from opponents. To study emotional feelings and expressions in negotiation dialogue, \citet{chawla2021towards} explore the prediction of two important subjective goals, including outcome satisfaction and partner perception. \citet{DBLP:conf/acl/LiuZDSLYJH20} provide explicit modeling on emotion transition engaged with pre-trained models (e.g., DialoGPT), to support help-seeker. Further, \citet{dutt2020keeping} propose a facing act modeling under the persuasive discussion scenarios. \citet{mishra2022pepds} utilize a reinforcement learning framework to engage emotion in the persuasive message. 

\subsubsection{Behavior Modeling}

Behavior modeling refers to detecting and predicting opponents' behaviors during the negotiation process. For example, fine-grained dialogue act labels are provided in the Craigslist dataset~\cite{he2018decoupling}, to help track the behaviors of buyers and sellers.  \citet{zhang2020learningbebavior} propose an opposite behavior modeling framework to estimate opposite action using DQN-based policy learning. \citet{chawla2021exploring} explore early prediction between negotiators for the outcomes. \citet{tran2022ask} leverage dialogue acts to identify optimal strategies to persuade humans for donation.


% related paper: Learning Goal-oriented Dialogue Policy with opposite Agent Awareness~\citet{zhang2020learningbebavior}




% Paper 1: Improving Dialog Systems for Negotiation with Personality Modeling~\cite{yang2021improving}:  Inspired by the idea of a theory of mind (ToM) into machines. we introduce a probabilistic formulation to encapsulate the opponent's personality type during both learning and inference.
% negotiation is task requires a combination of good comminication skills and strategic reasoning capabilities.
% MDP-based method RL
% first-order ToM policy with explicit/implicit variance.

% Paper 2: Opponent Modeling in Negotiation Dialogues
% by Related Data Adaptation~\cite{chawla2022opponent}: 
% Opponent modeling is the task of inferring another party’s mental state within the context of social interactions.
% In a multi-issue negotiation, it involves inferring the relative importance that the opponent assigns to each issue under discussion, which is crucial for finding high-value deals.
% we propose a ranker for identifying these priorities from
% negotiation dialogues. We further devise ways to adapt related data sources for this task to provide more explicit supervision for incorporating the opponent’s preferences and offers,


% Paper 3: Keeping Up Appearances: Computational Modeling of Face Acts in
% Persuasion Oriented Discussions:  Modeling face and understanding its state changes throughout a conversation is critical to the study of maintenance of basic human needs in and through interaction. Grounded in the politeness theory of Brown and Levinson (1978), we propose a
% generalized framework for modeling face acts  in persuasion conversations, resulting in a reliable coding manual, an annotated corpus, and  computational models.  on the donation persuassion task.
% FaceAct: SPos+, SPos-, HPos+, HPos- SNeg+, SNeg-, HNeg+, HNeg- 


% Paper 4: Towards Emotion-Aware Agents For Negotiation. To advance the development of such agents, we explore the prediction of two important
% subjective goals in a negotiation – outcome satisfaction and
% partner perception. We study three degrees of emotion dimensions – emoticons, lexical, and contextual by leveraging affective lexicons and a state-of-the-art deep learning architecture.
% How humans negotiate has been extensively studied in multiple disciplines: Game Theory for identifying optimal behaviors [15], Psychology for understanding human decision-making [16], and Computer Science for building automated negotiation agents.
% Comprehensive emotion analysis.

% Paper 5: Exploiting Personal Characteristics of Debaters for
% Predicting Persuasiveness~\cite{alkhatib2020exploiting}.
% the personal characteristics of an argument’s source and audience
% have not yet been fully exploited toward automated persuasiveness prediction. In this paper, we model debaters’ prior beliefs, interests, and personality traits based on their previous activity, without dependence on explicit user profiles or questionnaire.




\subsection{Policy Learning}

Policy learning plays an important role in negotiation dialogue systems, by which the agent learns to choose a strategy and generate a response for the next step. Methods of policy learning can be roughly categorized into three types: \emph{reinforcement learning}, \emph{supervised learning}, and \emph{multitask learning}.



% Policy learning is an important procedure in the negotiation dialogue system, by which the agent learns to predict a policy or a strategy for negotiation, given the dialogue history and the final goal of this negotiation.
% There are typically three learning methods, supervised learning, reinforcement learning, and multitask learning.


\subsubsection{Reinforcement Learning}

Reinforcement learning (RL) is one of the most common frameworks chosen for policy learning. \citet{english2005learning} are the first to use RL techniques for negotiation dialogue systems. They employed a single-agent pattern to learn the policy of two opponents individually. But single-agent RL techniques are not well suited for concurrent learning where each agent is trained against a continuously
changing environment. Therefore, \citet{georgila2014single} further advances the framework with concurrent progress using multi-agent RL techniques, which simultaneously model two parties and provide a way to deal with multi-issues scenarios. Besides, \citet{keizer-etal-2017-evaluating} propose to learn the action of the target agents with a Q-learning reward function. They further propose a method based on hand-crafted rules and a method using Random Forest trained on a large human negotiation corpus from~\cite{afantenos2012modelling}.

Most recent works try to equip RL with deep learning techniques. For instance, \citet{zhang2020learningbebavior} propose OPPA, which lets the target agent behave given the system actions. The system actions are predicted and conditioned on the target agent's actions. The reward of the actions for the target agent is obtained by predicting a structured output given the whole dialogue.
%(e.g., the number of book or hat items obtained by the agent) or from real users. 
Besides, \citet{shi2021refine} use a modular framework containing a language model to generate responses, a response detector would automatically annotate the response with a negotiation strategy, and an RL-based reward function to assign a score to the strategy. Instead of the modular framework which separates policy learning and response generation, \citet{gao2021deepRL} propose an integrated framework with deep Q-learning, which includes multiple channel negotiation skills. It allows agents to leverage parameterized DQN to learn a comprehensive negotiation strategy that integrates linguistic communication skills and bidding strategies.

% \textbf{Refine and Imitate: Reducing Repetition and Inconsistency in Persuasion
% Dialogues via Reinforcement Learning and Human Demonstration} DialGAIL~\cite{shi2021refine} uses a language model to generate a response given the user utterance. Then a response detector would annotate the response with a persuasion strategy. The reward function assigns a reward to the persuasion strategy and  the reinforcement learning (RL) process to refine a baseline language model for better response generation given the reward.

% \textbf{Learning Goal-oriented Dialogue Policy with Opposite Agent Awareness}Instead of letting the target agent interact with a pre-defined environment as most RL methods do, OPPA~\cite{zhang2020learningbebavior} let the target agent behave given the system actions, which is predicted conditioned on the target agent actions. The reward of the actions of the target agent is obtained by predicting a structured output given the whole dialogue (e.g., the number of book or hat items obtained by the agent) or from real users.

% \textbf{Single-Agent vs. Multi-Agent Techniques for Concurrent
% Reinforcement Learning of Negotiation Dialogue Policies} Similiar to OPPA~\cite{zhang2020learning}, ~\cite{georgila2014single} learns the target agent and opponent agent simultaneously as well.

% \textbf{Evaluating Persuasion Strategies and Deep Reinforcement Learning
% methods for Negotiation Dialogue agents}~\cite{keizer2017evaluating} proposes an RL method to learn the action of the target agents to win a chess game. ~\cite{keizer2017evaluating} also proposes a mehtod based on hand-crafted rules and a method using Random Forest trained on a large human negotiation corpus from~\cite{afantenos2012modelling}.


\subsubsection{Supervised Learning}
 
Supervised learning (SL) is another popular paradigm  for policy learning. \cite{lewis2017deal} adopt a Seq2Seq model to learn what action should be taken by maximizing the likelihood of the training data. However, supervised learning only aims to mimic the average human behavior, so~\citet{he2018decoupling} propose to finetune the supervised model to directly optimize for a particular dialogue reward function, which is defined as i) the utility function of the final price for the buyer and seller ii) the difference between two agents’ utilities iii) the number of utterances in the dialogue. \citet{zhou2019augmenting} train a strategy predictor to predict whether a certain negotiation strategy occurred in the next utterance using supervised training. The system response would be generated conditioned on the user utterance, dialogue context, and the predicted negotiation strategy. In addition, \citet{joshi2021dialograph} incorporate a pragmatic strategies graph network with the seq2seq model to create an interpretable policy learning paradigm.  Recently,  \citet{dutt2021resper} propose a generalised
framework for identifying resisting strategies in persuasive negotiations using a pre-trained BERT model~\cite{devlin2019bert}.


% \textbf{Decoupling Strategy and Generation in Negotiation Dialogues}~\cite{he2020decoupling} adopts a Seq2Seq model to learn what action should be taken by maximizing the likelihood of the training data. However, supervised learning only aims to mimic the average human behavior, so~\citet{he2020decoupling} proposes to finetune the supervised model to directly optimize for a particular dialogue reward function, which is defined as i) the utility function of the final price for the buyer and seller ii) the difference between two agents’ utilities iii) the number of utterances in the dialogue.

% \textbf{AUGMENTING NON-COLLABORATIVE DIALOG SYSTEMS WITH EXPLICIT SEMANTIC AND STRATEGIC DIALOG HISTORY}~\cite{zhou2019augmenting} train a strategy predictor to predict whether a certain negotiation strategy occurred in the next utterance given current utterance and dialogue history using supervised training. The system response would be generated conditioned on the user utterance, dialogue context, and the predicted negotiation strategy.

% \textbf{Deal or No Deal? End-to-End Learning for Negotiation Dialogues}~\cite{lewis2017deal} trains a supervised model first, followed by finetuning this model with RL strategies.



\subsubsection{Multi-task Learning}

Multi-task learning aims to jointly train the system with several sub-tasks and finally achieve satisfactory performance. \citet{li2020end} propose an end-to-end framework that integrates several sub-tasks including intent and semantic slot classification,  response generation and filtering tasks in a Transformer-based pre-trained model. \citet{zhou2019augmenting} propose to jointly model both semantic and strategy history using finite state transducers (FSTs) with hierarchical neural models. \citet{chawla2022opponent} integrate a preference-guided response generation model with a ranker module to identify opponents' priority.

==> negotiation survey/6-evaluation_method.tex <==
\section{Evaluation}

We categorize the evaluation methods for negotiation dialogue systems into three types: goal-oriented metrics, game-based metrics and human evaluation.
Table~\ref{tab:metrics} lists the evaluation metrics that are introduced in our survey. 

\subsection{Goal-based Metrics}

Goal-oriented metrics mainly consider the agent's proximity to the goal from the perspective of strategy modeling, task fulfillment and sentence realization. \textit{Success Rate (SR)} is the most widely used, which measures how frequently an agent completes the task within their goals. A similar metric \textit{Prediction Accuracy (PA)} is to evaluate the agent's strategy predictions or the outcome of negotiations, such as macro or average F1 score~\cite{wang-etal-2019-persuasion,dutt2020keeping,chawla2021casino}. For those scenario-related tasks,
\citet{yamaguchi-etal-2021-dialogue} present a task where the model is required to label the human-human negotiation outcomes as either a success or a breakdown, including area under the curve (ROC-AUC), confusion matrix (CM), and average precision (AP).  \citet{DBLP:conf/naacl/KornilovaED22} propose a model-based evaluation based on Item Response Theory to analyze the effectiveness of persuasion on the audience.

In terms of language realization for negotiation dialogue,
\citet{DBLP:books/sp/15/HiraokaNSTN15} employ a predefined naturalness metric (a bigram overlap between the system responses and the ground-truth responses) as part of the reward to evaluate policies in cooperative persuasive dialogues.
%\citet{lewis2017deal} use perplexity to compare the model-generated responses with the ground-truth human sentences in multi-issue bargaining tasks.
Other classical metrics for evaluating the quality of response are also used, i.e., perplexity (PPL), BLEU-2, ROUGE-L, and BOW Embedding-based Extrema matching score~\cite{lewis2017deal}.

% \subsection{Automatic Evaluation}
% Several automatic evaluation metrics are used for the evaluation of negotiation dialogue systems.
% \citet{DBLP:books/sp/15/HiraokaNSTN15} employ naturalness (a bigram overlap between the system responses and the ground-truth responses) as part of the reward to evaluate policies in cooperative persuasive dialogues.
% \citet{lewis2017deal} use perplexity to compare the model generated responses with the ground-truth human sentences in multi-issue bargaining task. 
% \citet{DBLP:conf/acl/LiuZDSLYJH20} focus on providing emotional support in conversation, and employ NLG to produce the NL sentences as responses. They employ classical metrics for evaluating the quality of text, i.e., perplexity (PPL), BLEU-2, ROUGE-L, and BOW Embedding-based Extrema matching score.

% \citet{nouri-traum-2014-initiative} disclose the relationship between initiative behavior in negotiation dialogues, and propose an agent predicting the goal and the outcome of the negotiations based on the initiative-based features.
% They leverage a metric of average accuracy to evaluate the agent's predictions.
% \citet{wang-etal-2019-persuasion} present a task where a participant tries to persuade his/her counterpart to donate to charity. They use a classifier to predict the 10 possible strategies used in the persuasion, and employ accuracy as well as macro F1 to evaluate the classifier.
% Following this work, \citet{dutt2020keeping} view face as a public self-image as well as an important factor in dialogues, and propose a framework targeting at modeling the state change of face in the donation-related conversations. They transform the face act and donation outcome predictions into classifying tasks, and use mean accuracy as well as macro F1-score to evaluate the two aforementioned predictions.
% \citet{DBLP:conf/naacl/ChawlaRCLMG21} adopt average F1-score and joint-A in their designed task where agents act as campsite neighbors to bargain for necessities. They use average F1-score to see whether the dialogue agent has accurately produced the desired strategies, and use joint-A to measure the percentage of the  sentences that the agent predicts all the correct strategies.
% \citet{DBLP:conf/naacl/KornilovaED22} resort to Item Response Theory to analyze the effectiveness of the latent traits in persuasions. They construct a binary task for predicting whether persuasion is successful, and thus use accuracy to measure their built classifier.
% \citet{yamaguchi-etal-2021-dialogue} present a task where model is required to label the human-human negotiation outcomes as either a success or a breakdown. In their task, the conventional performance measurement for the classification problems are adopted to evaluate the model, including area under curve (ROC-AUC), confusion matrix (CM), and average precision (AP).

% The automatic evaluation metrics provide a quantitative perspective in evaluating the NL responses or the negotiation-related strategies predicted by the designed agents. 
% The researchers could derive such the metrics without manual efforts, and more importantly, are able to have an intuitive sense about the models' performance.  

\begin{table*}[ht]
\begin{center}
\small
\begin{tabular}{cc}
\toprule
    \makecell[c]{Goal-based \\ Metrics}  & \makecell[c]{SR, PA (\citeyear{nouri-traum-2014-initiative,wang-etal-2019-persuasion,dutt2020keeping,DBLP:conf/naacl/KornilovaED22}); Average F1 score (\citeyear{chawla2021casino}); \\ Macro F1 score (\citeyear{wang-etal-2019-persuasion,dutt2020keeping}); ROC-AUC, CM, AP (\citeyear{yamaguchi-etal-2021-dialogue});  Naturalness (\citeyear{DBLP:books/sp/15/HiraokaNSTN15}); \\ PPL, BLEU-2, ROUGE-L, Extrema (\citeyear{lewis2017deal})} \\ 
\midrule
    \makecell[c]{Game-based \\ Metrics} & \makecell[c]{WinRate, AvgVPs (\citeyear{keizer-etal-2017-evaluating}); Utility, Fairness, Length (\citeyear{he2018decoupling});\\ Average Sale-to-list Ratio, Task Completion Rate (\citeyear{zhou-etal-2019-dynamic})} \\ 
\midrule
    \makecell[c]{Human \\ Evaluation} & \makecell[c]{Agent satisfaction (\citeyear{DBLP:books/sp/15/HiraokaNSTN15, lewis2017deal}); Purchase decision, Correct response rate (\citeyear{DBLP:books/sp/15/HiraokaNSTN15}) \\ Achieved agreement rate, Pareto optimality rate (\citeyear{lewis2017deal}); Likert score (\citeyear{he2018decoupling})} \\ 
\bottomrule
\end{tabular}
\caption{Various Metrics used in the existing negotiation dialogues benchmarks.}
\label{tab:metrics}
\end{center}
\end{table*}

\subsection{Game-based Metrics}
Different from goal-oriented metrics, which focus on evaluating the accuracy of strategies or actions, game-based evaluation provides a user-centric perspective through multi-turn interactions. \citet{keizer-etal-2017-evaluating} measure the bots' negotiation strategies within the online game "Settlers of Catan" by proposing the metrics WinRate (the percentage of games won by the humans when playing with the bot opponents) and AvgVPs (the average number of victory points gained by the human players). \citet{he2018decoupling} present a task that two agents bargain to get the best deal using natural language. They use task-specific scores to test the performance of the agents, including utility (a score that is higher when the final price is closer to one agent's expected price), fairness (the difference between two agents' utilities), and length (the number of the sentences exchanged between the two agents).  \citet{zhou-etal-2019-dynamic} design a task where a seller and a buyer try to achieve a mutually acceptable price through a natural language negotiation. They adopt different metrics to evaluate the dialogue agent, i.e., average sale-to-list ratio 
%(the ratio that is between the final price paid by the buyer and the original price listed by the seller) 
and the task completion rate.
%(the percentage of the dialogues that both agents eventually accept a price). 
Besides, \citet{cheng2019evaluating} propose an adversarial attacking evaluation approach to test the robustness of negotiation systems.

%Due to the fact that automatic evaluation metrics mainly focus on assessing the accuracy of the strategies or actions that dialogue systems take in the process of negotiating, game-based evaluation is further used to provide a more precise evaluation of the negotiations. 

% \citet{keizer-etal-2017-evaluating} measure the bots' negotiation strategies within the online game "Settlers of Catan" by proposing the metrics WinRate (the percentage of games won by the humans when playing with the bot opponents) and AvgVPs (the average number of victory points gained by the human players). 

% \citet{DBLP:conf/emnlp/HeCBL18} present a task that two agents bargain to get the best deal using natural language. They use task-specific scores to test the performance of the agents, including utility (a score which is higher when the final price is closer to one agent's expected price), fairness (difference between two agents' utilities), and length (the number of the sentences exchanged between the two agents).

% Likewise, \citet{zhou-etal-2019-dynamic} design a task where a seller and a buyer try to achieve a mutually acceptable price through a natural language negotiation. They adopt different metrics to evaluate the dialogue agent, i.e., average sale-to-list ratio (the ratio that is between the final price paid by the buyer and the original price listed by the seller) and the task completion rate (the percentage of the dialogues that both agents eventually accept a price). 

% The game-based evaluation presents a quantitative perspective, focusing on the gains or losses when the agents negotiating in the games. 
 
\subsection{Human Evaluation}
To evaluate the users' satisfaction with the dialogue systems, human judgment is employed as a subjective evaluation of the generated output.
%In human evaluation, human annotators are asked to score generated responses along multiple dimensions of quality, such as satisfaction, comfort, and fluency, in the negotiations.
\citet{DBLP:books/sp/15/HiraokaNSTN15} use a dialogue system as the salesperson to bargain with the human customers and have the users annotate subjective customer satisfaction (a five-level score), the final decision of making a purchase (a binary number indicating whether persuasion is successful), and the correct response rate in the dialogues.
\citet{lewis2017deal} employ crowd-sourcing workers to highlight that essential information when bargaining with dialogue systems, covering the percentage of dialogues where both interlocutors finally achieve an agreement, and \emph{Pareto optimality}, i.e., the percentage of the Pareto optimal solutions in all the agreed deals. 
%(no alternative state that would make one agent better off without making the other agent worse off) in all the agreed deals.    
\citet{he2018decoupling} propose human likeness as a metric in evaluating how well the dialogue system is doing in a bargain. They ask workers to manually score the dialogue agent using a \emph{Likert} metric to judge whether the agent acts like a real human or not.
% \citet{DBLP:conf/acl/LiuZDSLYJH20} recruit Amazon Mechanical Turk (AMT) workers to provide qualitative feedback regarding the responses generated by the emotional support dialogue systems, including fluency (contextual Coherence), identification (how deeply identify the users' problems), comforting (levels of comfort that is offered by the agent), suggestion (how helpful the suggestions are), and overall (choose the preferable one from two comparative agents).    

% Owing to the manual annotation efforts, human evaluation is naturally more costly compared to automatic evaluation, but more representative of the quality of the generated output.




==> negotiation survey/7-new_frontiers.tex <==
\section{New Frontiers and Challenges}
Previous sections summarize the prominent achievements of previous work in negotiation dialogue, including benchmarks, evaluation metrics and methodology. In this section, we will discuss some new frontiers which allow negotiation dialogue systems to be fit actual application needs and applied in real-world scenarios. 


\subsection{Multi-modal Negotiation Dialogue}
Existing research works in negotiation dialogue only consider text format as inputs and outputs. However, humans tend to perceive the world in multi-modal patterns, not only text but also audio and visual information. For example, the facial expression and emotions of participants in a negotiation dialogue could be important cues for making negotiation decisions. Further work can consider adding this non-verbal information into the negotiation process.


\subsection{Multi-Party Negotiation Dialogue}
Although some work sheds light on multi-party negotiation, most current negotiation dialogue benchmarks and methods predominantly focus on two-party settings. Therefore, multi-party negotiation dialogues are under-explored. Future work can consider collecting dialogues in multi-party negotiation scenarios, including \emph{General multi-party negotiation} and \emph{Team negotiation.} Specifically, \emph{General multi-party negotiation} is a type of bargaining where more than two parties negotiate toward an agreement. For example, next-year budget discussion with multiple department leaders in a large company. \emph{Team negotiation} is a team of people with different relationships and roles. It is normally associated with large business deals and highlights the significance of relationships between multi-parties. There could be several roles, including leader, recorder, and examiner, in a negotiation team~\cite{halevy2008team}.

\subsection{Cross-Culture \& Multi-lingual Negotiation Dialogue}
Existing negotiation dialogue benchmarks overwhelmingly focused on English while leaving other languages and backgrounds under exploration. With the acceleration of globalization, a dialogue involving individuals from different culture backgrounds participants becomes increasingly important and necessary. That is, there is an urgent need to provide people with a negotiation dialogue system with different cultures and multi-lingual. Further works can consider incorporating multi-lingual utterances and social norms among different countries into negotiation dialogue benchmarks.

%For example, crossed arms while standing is a sign of defensiveness and protection


\subsection{Negotiation Dialogue in Real-world Scenarios}
As discussed in Section~\ref{datasetsection}, previous works have already proposed many negotiation dialogue benchmarks in various scenarios. However, we notice that most of these benchmarks are artefacts through human crowd-sourcing. Participants are often invited to play specific roles in the negotiation dialogue. The resulting dialogues may not perfectly reflect the negotiations in real-world scenarios (e.g., politics, business). Therefore, it could be a promising research direction to collect real negotiation dialogues. For example, one could collect recorded business meetings or phone calls. 


% effective methods to resolve the limited resource problem.




% While previous sections mainly point out new scenarios or settings as new research directions, we also argue that the limited resource problem hinders the development of negotiation dialogue system. Although many benchmarks are proposed to facilitate the research of negotiation dialogue, most of them are artefact through human crowd-sourcing. Dialogue in real-scenarios are difficult to collect, especially in some privacy-sensitive domains 

==> negotiation survey/8-conclusion.tex <==
\section{Conclusion}


This paper presents the first systematic review on the progress of the negotiation dialogue system. We thoroughly summarize the existing works, which cover various domains and highlight their challenges respectively. Besides, we summarize currently available benchmarks, evaluations, and methodologies. In addition, we shed light on some new trends in this research field. We hope this survey can facilitate future research on negotiation dialogue systems.

==> negotiation survey/9-related_work.tex <==
\section{Related Work}

other relevant survey work on dialogue systems.

==> negotiation survey/abstract.tex <==
\begin{abstract}

Negotiation is one of the crucial abilities in human communication, and there has been a resurgent research interest in negotiation dialogue systems recently, which goal is to empower intelligent agents with such ability that can efficiently help humans resolve conflicts or reach beneficial agreements. Although there have been many explorations in negotiation dialogue systems, a systematic review of this task has to date remained notably absent. To this end, we aim to fill this gap by reviewing contemporary studies in the emerging field of negotiation dialogue systems, covering benchmarks, evaluations, and methodologies. Furthermore, we also discuss potential future directions, including multi-modal, multi-party, and cross-cultural negotiation scenarios. Our goal is to provide the community with a systematic overview of negotiation dialogue systems and to inspire future research.


% Negotiation is a crucial ability in daily communication. The research goal of negotiation dialogue system is to build intelligent agents that can can communicate with humans to more efficiently resolve their conflicts and reaching mutually beneficial agreements. Although negotiation dialogue systems have gained traction recently, a systematic review for this task has to date remained noticeably absent. To this end, we take the first step and present a survey on this task. Specifically, we review contemporary studies in the emerging field of negotiation dialogue systems, from benchmarks, evaluations, and methodologies. Furthermore, we discuss some future directions, including multi-modal, multi-party and cross-culture negotiation scenarios. We hope that this first survey of negotiation dialogue system can provide the community with a quick access and a general picture to this task and motivate future researches.


%Negotiation dialogue system is a non-collaborative task, which requires complex communication and strategy skills between speakers. Recently, the promising achievements in both dialogue systems and machine learning techniques dramatically lead this task to a new landscape. However, there still remains a lack of a comprehensive survey for this task. To this end, we take the first step and present a survey on the research field. Specifically, we categorize current work from methodology, application scenarios and dataset. Furthermore, we discuss some potential directions and challenges. The collected resources for negotiaion dialogue are available here.
%\footnote{\url{https://github.com/zhanhl316/negotiation-dialogue-survey}}

\end{abstract}

==> negotiation survey/macros.tex <==
\newcommand{\eg}{e.g., }
\newcommand{\ie}{i.e., }
\newcommand{\PR}{\hbox{Pr}}



\newcommand{\heart}{\ensuremath\heartsuit}
\newcommand{\diamondsmall}{\ensuremath\diamondsuit}


\newcommand\noteIZ[1]{\marginpar[\scriptsize
\textcolor{red}{\hfill #1}]{\scriptsize \textcolor{red}{#1}}}

\newcommand\noteHZ[1]{\marginpar[\scriptsize
\textcolor{blue}{\hfill #1}]{\scriptsize \textcolor{blue}{#1}}}

\newcommand\noteRH[1]{\marginpar[\scriptsize
\textcolor{red}{\hfill #1}]{\scriptsize \textcolor{red}{#1}}}


\newcommand{\haolan}[1]{\textcolor{blue}{#1}}
\newcommand{\Reza}[1]{\textcolor{green}{#1}}
\newcommand{\Lizhen}[1]{\textcolor{red}{#1}}
